Lifelong Continual Learning for Anomaly Detection: New Challenges, Perspectives, and Insights

Anomaly detection is of paramount importance in many real-world domains, characterized by evolving behavior. Lifelong learning represents an emerging trend, answering the need for machine learning models that continuously adapt to new challenges in dynamic environments while retaining past knowledge. However, limited efforts are dedicated to building foundations for lifelong anomaly detection, which provides intrinsically different challenges compared to the more widely explored classification setting. In this paper, we face this issue by exploring, motivating, and discussing lifelong anomaly detection, trying to build foundations for its wider adoption. First, we explain why lifelong anomaly detection is relevant, defining challenges and opportunities to design anomaly detection methods that deal with lifelong learning complexities. Second, we characterize learning settings and a scenario generation procedure that enables researchers to experiment with lifelong anomaly detection using existing datasets. Third, we perform experiments with popular anomaly detection methods on proposed lifelong scenarios, emphasizing the gap in performance that could be gained with the adoption of lifelong learning. Overall, we conclude that the adoption of lifelong anomaly detection is important to design more robust models that provide a comprehensive view of the environment, as well as simultaneous adaptation and knowledge retention.

==> tables/guide_table.tex <==
\begin{tabular}{lrrr}
     &  \\
     & 
\end{tabular}

==> tables/results-cumulative.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr} \\ 
\toprule
 & \multicolumn{3}{c}{IF} & \multicolumn{3}{c}{LOF} & \multicolumn{3}{c}{COPOD} & \multicolumn{3}{c}{OC-SVM} & \multicolumn{3}{c}{VAE} \\ 
& AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT \\ 
\midrule
 energy-CC-10c-1k0s & 0.64 (0.82) & -0.29 & 0.61 & 0.71 (0.95) & -0.31 & 0.81 & 0.85 (0.89) & -0.07 & 0.90 & 0.76 (0.83) & -0.22 & 0.84 & 0.75 (0.77) & -0.21 & 0.81 \\ 
 energy-CC-20c-1k0s & 0.56 (?) & -0.33 & 0.57 & 0.67 (?) & -0.32 & 0.81 & 0.79 (?) & -0.11 & 0.88 & 0.71 (?) & -0.24 & 0.86 & 0.70 (?) & -0.24 & 0.85 \\ 
 energy-CC-5c-1k0s & 0.69 (?) & -0.38 & 0.64 & 0.77 (?) & -0.33 & 0.81 & 0.87 (?) & -0.13 & 0.88 & 0.82 (?) & -0.24 & 0.91 & 0.81 (?) & -0.25 & 0.91 \\ 
 energy-CR-10c-1k0s & 0.65 (0.78) & -0.40 & 0.53 & 0.70 (0.96) & -0.35 & 0.73 & 0.91 (0.89) & -0.09 & 0.86 & 0.75 (0.85) & -0.29 & 0.71 & ? (0.78) & ? & ? \\ 
 energy-CR-20c-1k0s & 0.56 (?) & -0.44 & 0.53 & 0.68 (?) & -0.35 & 0.72 & 0.86 (?) & -0.14 & 0.88 & 0.70 (?) & -0.33 & 0.74 & 0.69 (?) & -0.34 & 0.74 \\ 
 energy-CR-5c-1k0s & 0.74 (?) & -0.33 & 0.55 & 0.84 (?) & -0.23 & 0.54 & 0.91 (?) & -0.09 & 0.81 & 0.87 (?) & -0.17 & 0.64 & 0.86 (?) & -0.19 & 0.65 \\ 
 energy-R-10c-1k0s & 0.59 (0.75) & -0.46 & 0.56 & 0.66 (0.97) & -0.41 & 0.70 & 0.89 (0.87) & -0.11 & 0.87 & 0.69 (0.84) & -0.37 & 0.70 & ? (0.76) & ? & ? \\ 
 energy-R-20c-1k0s & 0.55 (?) & -0.45 & 0.54 & 0.66 (?) & -0.37 & 0.62 & 0.87 (?) & -0.12 & 0.87 & 0.68 (?) & -0.34 & 0.65 & 0.67 (?) & -0.36 & 0.64 \\ 
 energy-R-5c-1k0s & 0.71 (?) & -0.38 & 0.61 & 0.75 (?) & -0.37 & 0.59 & 0.91 (?) & -0.11 & 0.85 & 0.80 (?) & -0.29 & 0.67 & 0.80 (?) & -0.28 & 0.67 \\ 
 nsl-kdd-CC-10c-1k0s & 0.77 (0.93) & -0.23 & 0.87 & 0.59 (0.89) & -0.38 & 0.62 & 0.55 (0.88) & -0.15 & 0.37 & 0.74 (0.78) & -0.26 & 0.89 & 0.73 (0.83) & -0.28 & 0.88 \\ 
 nsl-kdd-CC-20c-3k0s & 0.69 (?) & -0.32 & 0.80 & 0.57 (?) & -0.41 & 0.55 & 0.49 (?) & -0.10 & 0.36 & 0.69 (?) & -0.33 & 0.86 & 0.69 (?) & -0.32 & 0.87 \\ 
 nsl-kdd-CC-20c-5ks & 0.68 (?) & -0.32 & 0.77 & 0.62 (?) & -0.33 & 0.56 & 0.54 (?) & -0.14 & 0.43 & 0.67 (?) & -0.36 & 0.85 & 0.67 (?) & -0.35 & 0.85 \\ 
 nsl-kdd-CC-3c-5k0s & ? (?) & ? & ? & ? (?) & ? & ? & ? (?) & ? & ? & ? (?) & ? & ? & 0.82 (?) & -0.32 & 0.80 \\ 
 nsl-kdd-CC-5c-1ks & 0.87 (?) & -0.20 & 0.82 & 0.77 (?) & -0.28 & 0.72 & 0.85 (?) & -0.20 & 0.73 & 0.88 (?) & -0.18 & 1.00 & 0.89 (?) & -0.17 & 0.99 \\ 
 nsl-kdd-CC-5c-3k0s & 0.88 (?) & -0.15 & 0.90 & 0.61 (?) & -0.47 & 0.56 & 0.69 (?) & -0.01 & 0.37 & 0.80 (?) & -0.27 & 0.93 & 0.82 (?) & -0.25 & 0.89 \\ 
 nsl-kdd-CR-10c-1k0s & 0.84 (0.90) & -0.19 & 0.72 & 0.57 (0.89) & -0.44 & 0.60 & 0.53 (0.85) & -0.14 & 0.38 & 0.82 (0.84) & -0.22 & 0.75 & 0.80 (0.87) & -0.24 & 0.73 \\ 
 nsl-kdd-CR-10c-3k0s & 0.80 (?) & -0.23 & 0.69 & 0.58 (?) & -0.44 & 0.51 & 0.43 (?) & -0.11 & 0.50 & 0.81 (?) & -0.23 & 0.75 & ? (?) & ? & ? \\ 
 nsl-kdd-CR-20c-3k0s & 0.73 (?) & -0.29 & 0.73 & 0.58 (?) & -0.42 & 0.55 & 0.48 (?) & -0.10 & 0.39 & 0.73 (?) & -0.30 & 0.78 & 0.73 (?) & -0.28 & 0.76 \\ 
 nsl-kdd-CR-20c-5ks & 0.70 (?) & -0.28 & 0.72 & 0.60 (?) & -0.37 & 0.54 & 0.52 (?) & -0.13 & 0.44 & 0.75 (?) & -0.23 & 0.73 & 0.73 (?) & -0.25 & 0.73 \\ 
 nsl-kdd-CR-3c-5k0s & 0.84 (?) & -0.32 & 0.36 & 0.59 (?) & -0.41 & 0.62 & 0.58 (?) & -0.22 & 0.25 & 0.84 (?) & -0.31 & 0.34 & 0.83 (?) & -0.33 & 0.34 \\ 
 nsl-kdd-CR-5c-1ks & 0.88 (?) & -0.18 & 0.57 & 0.79 (?) & -0.27 & 0.37 & 0.89 (?) & -0.13 & 0.45 & 0.87 (?) & -0.20 & 0.69 & 0.87 (?) & -0.20 & 0.69 \\ 
 nsl-kdd-CR-5c-3k0s & 0.86 (?) & -0.20 & 0.67 & 0.71 (?) & -0.35 & 0.52 & 0.53 (?) & 0.04 & 0.43 & 0.85 (?) & -0.23 & 0.64 & 0.84 (?) & -0.22 & 0.63 \\ 
 nsl-kdd-R-10c-1k0s & 0.86 (0.96) & -0.17 & 0.84 & 0.55 (0.92) & -0.51 & 0.56 & 0.77 (0.95) & -0.18 & 0.73 & 0.87 (0.95) & -0.15 & 0.89 & 0.87 (0.94) & -0.15 & 0.88 \\ 
 nsl-kdd-R-10c-3k0s & 0.87 (?) & -0.15 & 0.85 & 0.46 (?) & -0.60 & 0.53 & 0.62 (?) & -0.07 & 0.61 & 0.87 (?) & -0.15 & 0.89 & ? (?) & ? & ? \\ 
 nsl-kdd-R-20c-3k0s & 0.85 (?) & -0.16 & 0.81 & 0.63 (?) & -0.34 & 0.55 & 0.59 (?) & -0.11 & 0.56 & 0.88 (?) & -0.13 & 0.84 & 0.86 (?) & -0.15 & 0.85 \\ 
 nsl-kdd-R-20c-5ks & 0.85 (?) & -0.16 & 0.82 & 0.63 (?) & -0.35 & 0.52 & 0.74 (?) & -0.08 & 0.67 & 0.88 (?) & -0.13 & 0.85 & 0.87 (?) & -0.14 & 0.86 \\ 
 nsl-kdd-R-3c-5k0s & 0.91 (?) & -0.16 & 0.85 & 0.68 (?) & -0.44 & 0.49 & 0.69 (?) & -0.10 & 0.48 & 0.90 (?) & -0.17 & 0.66 & 0.90 (?) & -0.18 & 0.76 \\ 
 nsl-kdd-R-5c-1ks & 0.90 (?) & -0.15 & 0.67 & 0.84 (?) & -0.21 & 0.77 & 1.00 (?) & -0.01 & 0.99 & 0.89 (?) & -0.16 & 0.91 & 0.92 (?) & -0.12 & 0.90 \\ 
 nsl-kdd-R-5c-3k0s & 0.92 (?) & -0.12 & 0.86 & 0.47 (?) & -0.71 & 0.41 & 0.77 (?) & -0.05 & 0.67 & 0.87 (?) & -0.19 & 0.86 & 0.87 (?) & -0.18 & 0.80 \\ 
 unsw-CC-10c-1k0s & 0.55 (0.70) & -0.39 & 0.57 & 0.75 (0.90) & -0.25 & 0.67 & 0.47 (0.64) & -0.15 & 0.40 & 0.72 (0.80) & -0.28 & 0.68 & 0.65 (?) & -0.35 & 0.66 \\ 
 unsw-CR-10c-1k0s & 0.51 (0.69) & -0.54 & 0.56 & 0.59 (0.91) & -0.47 & 0.55 & 0.49 (0.56) & -0.29 & 0.36 & 0.66 (0.78) & -0.42 & 0.50 & 0.63 (?) & -0.46 & 0.47 \\ 
 unsw-CR-10c-3k0s & 0.60 (?) & -0.41 & 0.50 & 0.67 (?) & -0.38 & 0.49 & 0.48 (?) & -0.24 & 0.24 & 0.73 (?) & -0.31 & 0.56 & 0.72 (?) & -0.32 & 0.51 \\ 
 unsw-R-10c-1k0s & 0.53 (0.67) & -0.51 & 0.46 & 0.62 (0.86) & -0.42 & 0.51 & 0.70 (0.61) & -0.23 & 0.54 & 0.54 (0.58) & -0.49 & 0.42 & 0.54 (?) & -0.52 & 0.41 \\ 
 unsw-R-10c-3k0s & 0.53 (?) & -0.45 & 0.45 & 0.60 (?) & -0.42 & 0.46 & 0.60 (?) & -0.18 & 0.44 & 0.55 (?) & -0.44 & 0.46 & 0.56 (?) & -0.46 & 0.44 \\ 
 wind-CC-10c-1k0s & 0.80 (0.87) & -0.08 & 0.75 & 0.59 (0.95) & -0.46 & 0.58 & 0.86 (0.86) & -0.05 & 0.88 & 0.74 (0.84) & -0.27 & 0.74 & 0.74 (?) & -0.27 & 0.75 \\ 
 wind-CR-10c-1k0s & 0.76 (0.86) & -0.21 & 0.67 & 0.60 (0.97) & -0.48 & 0.51 & 0.93 (0.90) & -0.07 & 0.86 & 0.72 (0.88) & -0.34 & 0.61 & 0.73 (?) & -0.33 & 0.58 \\ 
 wind-R-10c-1k0s & 0.72 (0.90) & -0.29 & 0.66 & 0.59 (0.98) & -0.50 & 0.54 & 0.93 (0.91) & -0.07 & 0.89 & 0.73 (0.91) & -0.32 & 0.65 & 0.79 (?) & -0.25 & 0.66 \\ 
\bottomrule
\end{tabular} \\ 


==> tables/results-know-it-all.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr} \\ 
\toprule
 & \multicolumn{3}{c}{IF} & \multicolumn{3}{c}{LOF} & \multicolumn{3}{c}{COPOD} & \multicolumn{3}{c}{OC-SVM} & \multicolumn{3}{c}{VAE} \\ 
& AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT \\ 
\midrule
 energy-CC-10c-1k0s & 0.64 (0.76) & -0.29 & 0.61 & 0.71 (0.94) & -0.31 & 0.81 & 0.85 (0.88) & -0.07 & 0.90 & 0.76 (0.81) & -0.22 & 0.84 & 0.75 (0.75) & -0.21 & 0.81 \\ 
 energy-CC-20c-1k0s & 0.56 (0.60) & -0.33 & 0.57 & 0.67 (0.92) & -0.32 & 0.81 & 0.79 (0.78) & -0.11 & 0.88 & 0.71 (0.74) & -0.24 & 0.86 & 0.70 (0.72) & -0.24 & 0.85 \\ 
 energy-CC-5c-1k0s & 0.69 (0.82) & -0.38 & 0.64 & 0.77 (0.97) & -0.33 & 0.81 & 0.87 (0.86) & -0.13 & 0.88 & 0.82 (0.92) & -0.24 & 0.91 & 0.81 (0.84) & -0.25 & 0.91 \\ 
 energy-CR-10c-1k0s & 0.65 (?) & -0.40 & 0.53 & 0.70 (?) & -0.35 & 0.73 & 0.91 (?) & -0.09 & 0.86 & 0.75 (?) & -0.29 & 0.71 & ? (?) & ? & ? \\ 
 energy-CR-20c-1k0s & 0.56 (0.61) & -0.44 & 0.53 & 0.68 (0.94) & -0.35 & 0.72 & 0.86 (0.78) & -0.14 & 0.88 & 0.70 (0.77) & -0.33 & 0.74 & 0.69 (0.71) & -0.34 & 0.74 \\ 
 energy-CR-5c-1k0s & 0.74 (0.81) & -0.33 & 0.55 & 0.84 (0.98) & -0.23 & 0.54 & 0.91 (0.92) & -0.09 & 0.81 & 0.87 (0.93) & -0.17 & 0.64 & 0.86 (0.91) & -0.19 & 0.65 \\ 
 energy-R-10c-1k0s & 0.59 (?) & -0.46 & 0.56 & 0.66 (?) & -0.41 & 0.70 & 0.89 (0.84) & -0.11 & 0.87 & 0.69 (?) & -0.37 & 0.70 & ? (?) & ? & ? \\ 
 energy-R-20c-1k0s & 0.55 (0.59) & -0.45 & 0.54 & 0.66 (0.94) & -0.37 & 0.62 & 0.87 (0.78) & -0.12 & 0.87 & 0.68 (0.76) & -0.34 & 0.65 & 0.67 (0.66) & -0.36 & 0.64 \\ 
 energy-R-5c-1k0s & 0.71 (0.82) & -0.38 & 0.61 & 0.75 (0.98) & -0.37 & 0.59 & 0.91 (0.89) & -0.11 & 0.85 & 0.80 (0.89) & -0.29 & 0.67 & 0.80 (0.77) & -0.28 & 0.67 \\ 
 nsl-kdd-CC-10c-1k0s & 0.77 (0.93) & -0.23 & 0.87 & 0.59 (0.84) & -0.38 & 0.62 & 0.55 (0.89) & -0.15 & 0.37 & 0.74 (0.77) & -0.26 & 0.89 & 0.73 (0.80) & -0.28 & 0.88 \\ 
 nsl-kdd-CC-20c-3k0s & 0.69 (?) & -0.32 & 0.80 & 0.57 (?) & -0.41 & 0.55 & 0.49 (?) & -0.10 & 0.36 & 0.69 (?) & -0.33 & 0.86 & 0.69 (?) & -0.32 & 0.87 \\ 
 nsl-kdd-CC-20c-5ks & 0.68 (?) & -0.32 & 0.77 & 0.62 (?) & -0.33 & 0.56 & 0.54 (?) & -0.14 & 0.43 & 0.67 (?) & -0.36 & 0.85 & 0.67 (?) & -0.35 & 0.85 \\ 
 nsl-kdd-CC-3c-5k0s & ? (?) & ? & ? & ? (?) & ? & ? & ? (?) & ? & ? & ? (?) & ? & ? & 0.82 (?) & -0.32 & 0.80 \\ 
 nsl-kdd-CC-5c-1ks & 0.87 (?) & -0.20 & 0.82 & 0.77 (?) & -0.28 & 0.72 & 0.85 (?) & -0.20 & 0.73 & 0.88 (?) & -0.18 & 1.00 & 0.89 (?) & -0.17 & 0.99 \\ 
 nsl-kdd-CC-5c-3k0s & 0.88 (?) & -0.15 & 0.90 & 0.61 (?) & -0.47 & 0.56 & 0.69 (?) & -0.01 & 0.37 & 0.80 (?) & -0.27 & 0.93 & 0.82 (?) & -0.25 & 0.89 \\ 
 nsl-kdd-CR-10c-1k0s & 0.84 (0.89) & -0.19 & 0.72 & 0.57 (0.84) & -0.44 & 0.60 & 0.53 (0.87) & -0.14 & 0.38 & 0.82 (0.83) & -0.22 & 0.75 & 0.80 (0.91) & -0.24 & 0.73 \\ 
 nsl-kdd-CR-10c-3k0s & 0.80 (0.84) & -0.23 & 0.69 & 0.58 (0.89) & -0.44 & 0.51 & 0.43 (0.76) & -0.11 & 0.50 & 0.81 (0.82) & -0.23 & 0.75 & ? (?) & ? & ? \\ 
 nsl-kdd-CR-20c-3k0s & 0.73 (?) & -0.29 & 0.73 & 0.58 (?) & -0.42 & 0.55 & 0.48 (?) & -0.10 & 0.39 & 0.73 (?) & -0.30 & 0.78 & 0.73 (?) & -0.28 & 0.76 \\ 
 nsl-kdd-CR-20c-5ks & 0.70 (?) & -0.28 & 0.72 & 0.60 (?) & -0.37 & 0.54 & 0.52 (?) & -0.13 & 0.44 & 0.75 (?) & -0.23 & 0.73 & 0.73 (?) & -0.25 & 0.73 \\ 
 nsl-kdd-CR-3c-5k0s & 0.84 (?) & -0.32 & 0.36 & 0.59 (?) & -0.41 & 0.62 & 0.58 (?) & -0.22 & 0.25 & 0.84 (?) & -0.31 & 0.34 & 0.83 (?) & -0.33 & 0.34 \\ 
 nsl-kdd-CR-5c-1ks & 0.88 (?) & -0.18 & 0.57 & 0.79 (?) & -0.27 & 0.37 & 0.89 (?) & -0.13 & 0.45 & 0.87 (?) & -0.20 & 0.69 & 0.87 (?) & -0.20 & 0.69 \\ 
 nsl-kdd-CR-5c-3k0s & 0.86 (?) & -0.20 & 0.67 & 0.71 (?) & -0.35 & 0.52 & 0.53 (?) & 0.04 & 0.43 & 0.85 (?) & -0.23 & 0.64 & 0.84 (?) & -0.22 & 0.63 \\ 
 nsl-kdd-R-10c-1k0s & 0.86 (0.95) & -0.17 & 0.84 & 0.55 (0.90) & -0.51 & 0.56 & 0.77 (0.94) & -0.18 & 0.73 & 0.87 (0.95) & -0.15 & 0.89 & 0.87 (0.93) & -0.15 & 0.88 \\ 
 nsl-kdd-R-10c-3k0s & 0.87 (?) & -0.15 & 0.85 & 0.46 (?) & -0.60 & 0.53 & 0.62 (?) & -0.07 & 0.61 & 0.87 (?) & -0.15 & 0.89 & ? (?) & ? & ? \\ 
 nsl-kdd-R-20c-3k0s & 0.85 (?) & -0.16 & 0.81 & 0.63 (?) & -0.34 & 0.55 & 0.59 (?) & -0.11 & 0.56 & 0.88 (?) & -0.13 & 0.84 & 0.86 (?) & -0.15 & 0.85 \\ 
 nsl-kdd-R-20c-5ks & 0.85 (?) & -0.16 & 0.82 & 0.63 (?) & -0.35 & 0.52 & 0.74 (?) & -0.08 & 0.67 & 0.88 (?) & -0.13 & 0.85 & 0.87 (?) & -0.14 & 0.86 \\ 
 nsl-kdd-R-3c-5k0s & 0.91 (?) & -0.16 & 0.85 & 0.68 (?) & -0.44 & 0.49 & 0.69 (?) & -0.10 & 0.48 & 0.90 (?) & -0.17 & 0.66 & 0.90 (?) & -0.18 & 0.76 \\ 
 nsl-kdd-R-5c-1ks & 0.90 (?) & -0.15 & 0.67 & 0.84 (?) & -0.21 & 0.77 & 1.00 (?) & -0.01 & 0.99 & 0.89 (?) & -0.16 & 0.91 & 0.92 (?) & -0.12 & 0.90 \\ 
 nsl-kdd-R-5c-3k0s & 0.92 (?) & -0.12 & 0.86 & 0.47 (?) & -0.71 & 0.41 & 0.77 (?) & -0.05 & 0.67 & 0.87 (?) & -0.19 & 0.86 & 0.87 (?) & -0.18 & 0.80 \\ 
 unsw-CC-10c-1k0s & 0.55 (0.70) & -0.39 & 0.57 & 0.75 (0.91) & -0.25 & 0.67 & 0.47 (0.64) & -0.15 & 0.40 & 0.72 (0.78) & -0.28 & 0.68 & 0.65 (0.88) & -0.35 & 0.66 \\ 
 unsw-CR-10c-1k0s & 0.51 (?) & -0.54 & 0.56 & 0.59 (?) & -0.47 & 0.55 & 0.49 (?) & -0.29 & 0.36 & 0.66 (?) & -0.42 & 0.50 & 0.63 (0.62) & -0.46 & 0.47 \\ 
 unsw-CR-10c-3k0s & 0.60 (0.59) & -0.41 & 0.50 & 0.67 (0.85) & -0.38 & 0.49 & 0.48 (?) & -0.24 & 0.24 & 0.73 (0.79) & -0.31 & 0.56 & 0.72 (?) & -0.32 & 0.51 \\ 
 unsw-R-10c-1k0s & 0.53 (0.62) & -0.51 & 0.46 & 0.62 (?) & -0.42 & 0.51 & 0.70 (0.59) & -0.23 & 0.54 & 0.54 (?) & -0.49 & 0.42 & 0.54 (0.63) & -0.52 & 0.41 \\ 
 unsw-R-10c-3k0s & 0.53 (0.44) & -0.45 & 0.45 & 0.60 (?) & -0.42 & 0.46 & 0.60 (0.52) & -0.18 & 0.44 & 0.55 (?) & -0.44 & 0.46 & 0.56 (?) & -0.46 & 0.44 \\ 
 wind-CC-10c-1k0s & 0.80 (0.85) & -0.08 & 0.75 & 0.59 (0.94) & -0.46 & 0.58 & 0.86 (0.85) & -0.05 & 0.88 & 0.74 (0.83) & -0.27 & 0.74 & 0.74 (0.73) & -0.27 & 0.75 \\ 
 wind-CR-10c-1k0s & 0.76 (0.83) & -0.21 & 0.67 & 0.60 (0.96) & -0.48 & 0.51 & 0.93 (0.89) & -0.07 & 0.86 & 0.72 (0.86) & -0.34 & 0.61 & 0.73 (0.77) & -0.33 & 0.58 \\ 
 wind-R-10c-1k0s & 0.72 (0.89) & -0.29 & 0.66 & 0.59 (0.96) & -0.50 & 0.54 & 0.93 (0.87) & -0.07 & 0.89 & 0.73 (0.89) & -0.32 & 0.65 & 0.79 (0.73) & -0.25 & 0.66 \\ 
\bottomrule
\end{tabular} \\ 


==> tables/results-replay-with-current-batch.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrr} \\ 
\toprule
 & \multicolumn{3}{c}{IF} & \multicolumn{3}{c}{LOF} & \multicolumn{3}{c}{COPOD} & \multicolumn{3}{c}{OC-SVM} & \multicolumn{3}{c}{VAE} \\ 
& AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT & AUC & BWT & FWT \\ 
\midrule
 energy-CC-10c-1k0s & 0.82 & -0.06 & 0.64 & 0.95 & -0.01 & 0.78 & 0.89 & -0.01 & 0.89 & 0.83 & -0.04 & 0.85 & ? & ? & ? \\ 
 energy-CR-10c-1k0s & 0.79 & -0.13 & 0.51 & 0.96 & -0.01 & 0.64 & 0.89 & -0.04 & 0.83 & 0.85 & -0.06 & 0.77 & 0.83 & 0.09 & 0.68 \\ 
 energy-R-10c-1k0s & 0.75 & -0.18 & 0.57 & 0.97 & -0.02 & 0.61 & 0.87 & -0.06 & 0.83 & 0.84 & -0.07 & 0.76 & 0.76 & -0.08 & 0.70 \\ 
 nsl-kdd-CC-20c-5ks & 0.86 & -0.12 & 0.92 & 0.89 & -0.03 & 0.33 & 0.79 & 0.00 & 0.78 & 0.71 & -0.21 & 0.89 & 0.82 & -0.16 & 0.92 \\ 
 nsl-kdd-CR-20c-5ks & 0.81 & -0.09 & 0.82 & 0.88 & -0.02 & 0.39 & 0.72 & -0.02 & 0.62 & 0.79 & -0.11 & 0.74 & 0.81 & -0.11 & 0.78 \\ 
 nsl-kdd-R-20c-5ks & 0.95 & -0.03 & 0.92 & 0.90 & -0.01 & 0.34 & 0.92 & 0.04 & 0.84 & 0.93 & -0.03 & 0.86 & 0.92 & -0.02 & 0.86 \\ 
 unsw-CC-10c-3k0s & 0.50 & -0.05 & 0.35 & 0.83 & -0.00 & 0.32 & 0.43 & 0.00 & 0.29 & 0.56 & -0.02 & 0.54 & 0.53 & 0.06 & 0.37 \\ 
 unsw-CR-10c-3k0s & 0.69 & -0.01 & 0.45 & 0.89 & -0.01 & 0.39 & 0.67 & 0.00 & 0.30 & 0.82 & 0.01 & 0.57 & 0.57 & 0.06 & 0.48 \\ 
 unsw-R-10c-3k0s & 0.45 & -0.08 & 0.34 & 0.82 & -0.05 & 0.40 & 0.52 & -0.05 & 0.39 & 0.50 & -0.08 & 0.46 & 0.61 & 0.19 & 0.35 \\ 
 wind-CC-5c-15ks & 0.92 & -0.01 & 0.79 & 0.97 & -0.01 & 0.60 & 0.92 & -0.01 & 0.90 & 0.91 & -0.04 & 0.83 & 0.90 & 0.02 & 0.82 \\ 
 wind-CR-5c-15ks & 0.87 & -0.11 & 0.71 & 0.97 & -0.03 & 0.57 & 0.89 & -0.06 & 0.89 & 0.88 & -0.08 & 0.75 & 0.86 & -0.02 & 0.79 \\ 
 wind-R-5c-15ks & 0.91 & -0.05 & 0.68 & 0.98 & -0.02 & 0.52 & 0.91 & -0.06 & 0.89 & 0.91 & -0.06 & 0.72 & 0.90 & -0.03 & 0.71 \\ 
\bottomrule
\end{tabular} \\ 

